Deep Nets with Subsampling Layers Unwittingly Discard Useful Activations at Test-Time

Subsampling layers play a crucial role in deep nets by discarding a portion of an activation map to reduce its spatial dimensions. This encourages the deep net to learn higher-level representations. Contrary to this motivation, we hypothesize that the discarded activations are useful and can be incorporated on the fly to improve models' prediction. To validate our hypothesis, we propose a search and aggregate method to find useful activation maps to be used at test time. We applied our approach to the task of image classification and semantic segmentation. Extensive experiments over nine different architectures on multiple datasets show that our method consistently improves model test-time performance, complementing existing test-time augmentation techniques. Our code is available at https://github.com/ca-joe-yang/discard-in-subsampling.

==> tables/aggregate_cifar100.tex <==
\begin{table}[h!]
\centering
\small
\caption{\textbf{CIFAR100 image classification.}}
\label{table:aggregate_cifar100}
\captionsetup{singlelinecheck = false}

\begin{tabular}{ l c c c c c  c c c c } 
\toprule
{Model} & {Standard} & {$B=1$} & {$B=7$} & {$B=10$}\\

\midrule
{Resnet-20} & 68.83 & 69.28 & 69.15 & \\
{Resnet-50} & \\
{Resnet-101} & \\
{EfficientNet-B0} & \\
{EfficientNet-B1} & \\
{MobileNetV2-50} & \\
{ViT-tiny-p16-224} & \\
{MobileViTV2-50} & \\
{Swin-tiny-p4-w7-224} & \\
{SwinV2-tiny-w8-256} & \\ % Running time 20 min per P
 
\bottomrule
\end{tabular}
%}
\end{table}


==> tables/ensemble_city.tex <==
\begin{table}[!t]
\centering
\small
\captionsetup{singlelinecheck = false}

\begin{tabular}{ c c c c c c  c c c c c c c } 
\specialrule{.15em}{.05em}{.05em}
 & & & \multicolumn{3}{c}{Cityscapes} & \multicolumn{3}{c}{ADE20K} \\
\cmidrule(lr){4-6}
\cmidrule(lr){7-9}
Backbone & Decoder & {Flip} & {Baseline} & $B_{\texttt{Ours}}=4$  & $B_{\texttt{Ours}}=10$  & {Standard} & $B = 4$  & $B = 10$  \\
% \cmidrule(lr){3-6}
% \cmidrule(lr){7-10}

\midrule

MobileNet & FCN & & 71.19 & \underline{71.27} & \bf{71.83} & 19.55 & {\bf 19.57} & \underline{19.56} \\
MobileNet & FCN & \ding{51} & 71.69 & \underline{72.03} & \bf 72.10  & \underline{19.72} & \underline{19.72} & \bf 19.73 \\
MobileNet & DeepLab & & 75.32 & \underline{75.58} & \bf 75.60 & 33.92 & \underline{34.01} & \textbf{34.09} \\
MobileNet & DeepLab & \ding{51} & 75.56 & \underline{75.75} & \textbf{75.76} &  34.18 &  \underline{34.20} & {\bf 34.28} \\
ResNet-50 & FCN & & 72.35 & \underline{72.50} & {\bf 72.66} & 35.94 & \underline{36.12}  & {\bf 36.20} \\
ResNet-50 & FCN  & \ding{51} & 72.71 & \underline{72.88} & {\bf 72.97} &  36.31 & \underline{36.46} & {\bf 36.50}  \\
ResNet-50 & DeepLab & & {79.60} & \underline{79.72} & {\bf 79.73} & {42.72} & \underline{42.77} & {\bf 42.81}\\
ResNet-50 & DeepLab  & \ding{51} & {80.08} & {\bf 80.15} & \underline{80.09} & {43.02} & {\bf 43.07} & \underline{43.06} \\
MiT & SegFormer & & 76.54 & \underline{77.01} & {\bf 77.05} &37.41 & {\bf 37.68}  & \underline{37.67}  \\
MiT & SegFormer & \ding{51} & 76.84 & \underline{77.11} & {\bf 77.12} & 38.03 & {\bf 38.33} & \underline{38.28} \\


\specialrule{.15em}{.05em}{.05em}
\end{tabular}
\caption{\textbf{Cityscapes and ADE20K results.
} We consider various encoder backbones and decoders w/ and w/o our procedure and TTA. We report the mIoU score on both Cityscapes and ADE20K semantic segmentation. Our procedure makes improvements on all combinations of architectures in both datasets. We also show that ours can improve the results of horizontal flip (TTA), proofing the complementary between the approaches. 
}
\label{table:ensemble_city}
%}
\vspace{-0.1cm}
\end{table}


==> tables/ensemble_imagenet.tex <==
%\begin{table}[t]
\centering
%\small
\captionof{table}{\textbf{ImageNet results.} We compare our approach, with different budgets, to the standard test-time procedure. Overall, we observe improvements in all $B=4$ and $B=10$ settings.
}
%\vspace{-0.1cm}
\label{table:ensemble_imagenet}
\captionsetup{singlelinecheck = false}

\begin{tabular}{ l c c c c c  c c c c } 
\specialrule{.15em}{.05em}{.05em}
{Model} & {Standard} & {$B=4$} &  {$B=10$}\\
% \cmidrule(lr){3-6}
% \cmidrule(lr){7-10}
%\midrule
\hline
{Resnet-18} & 69.758 & \underline{70.018} & \bf 70.324 \\
{Resnet-50} & 80.384 & \underline{80.594} & \bf 80.804  \\
{Resnet-101} & 81.922 & \underline{82.182} & \bf 82.314\\
{EfficientNet} & 77.686 & \underline{77.792} & \bf 77.950  \\
% {EfficientNet-B1} & 78.796 & \underline{78.954} & \bf{79.132} \\
{MobileNet} & 65.940 & \underline{66.106} & \bf 66.274 \\
% {MobileNetv3-small-50} & 57.902 & 58.214 & & 58.132\\
%{ViT} & 75.466 & \underline{76.570} & \bf{76.578} \\
% {mViTV2-tiny} & 82.532 & & 82.612 \\
{MobileViT} & 70.148 & \underline{70.436} & \bf{70.656} \\
{Swin} & \underline{81.376} & {\bf 81.588} & {81.342} \\ %81.344
{SwinV2} & 81.818 & {\bf 82.034} & \underline{82.028} \\ % Running time 20 min per P
% {maxvit-tiny_rw_224}
% {deit3-small-p16-224} & 83.070 & 83.074\\
% {CvT} After BN
 
\specialrule{.15em}{.05em}{.05em}
\end{tabular}
%}
%\end{table}

% Resnet-18 69.756 70.014 70.310
% Resnet-50 80.384 80.606 80.826
% Resnet-101 81.924 82.234 82.344
% EfficientNet 77.692 77.794 77.914
% MobileNet 65.944 66.092 66.312
% ViT 75.466 75.778 76.214
% MobileViT 70.154 70.430 70.638
% Swin 81.374 81.590 81.630
% SwinV2 81.814 82.026 82.022

% {Resnet-18} & 69.756 & 70.038 & 70.248 & 70.322 & 70.264\\
% {Resnet-50} & 80.384 & 80.606 & 80.726 & 80.826 & 80.872 \\
% {Resnet-101} & 81.924 & 82.234 & 82.326 & 82.344 & 82.348\\
% {EfficientNet-B0} & 77.692 & 77.794 & 77.834 & 77.914 & 77.870 \\
% {EfficientNet-B1} & 78.796 & 78.954 & 79.078 & 79.132\\
% {MobileNetV2-50} & 65.944 & 66.036 & 66.250 & & 66.578 \\
% {MobileNetv3-small-50} & 57.902 & 58.214 & & 58.132\\
% {ViT-tiny-p16-224} & 75.454 & 76.268 & & 76.266 \\
% % {mViTV2-tiny} & 82.404 & & 82.508 \\
% {MobileViTV2-50} & 70.154 & 70.372 & & 70.804 \\
% {Swin-tiny-p4-w7-224} & 81.374 & 81.590 & & 81.630 \\
% {SwinV2-tiny-w8-256} & 81.814 & 82.100 & & 82.034 \\
